ReasonIR: Training Retrievers for Reasoning Tasks

We present ReasonIR-8B, the first retriever specifically trained for general reasoning tasks. Existing retrievers have shown limited gains on reasoning tasks, in part because existing training datasets focus on short factual queries tied to documents that straightforwardly answer them. We develop a synthetic data generation pipeline that, for each document, our pipeline creates a challenging and relevant query, along with a plausibly related but ultimately unhelpful hard negative. By training on a mixture of our synthetic data and existing public data, ReasonIR-8B achieves a new state-of-the-art of 29.9 nDCG@10 without reranker and 36.9 nDCG@10 with reranker on BRIGHT, a widely-used reasoning-intensive information retrieval (IR) benchmark. When applied to RAG tasks, ReasonIR-8B improves MMLU and GPQA performance by 6.4% and 22.6% respectively, relative to the closed-book baseline, outperforming other retrievers and search engines. In addition, ReasonIR-8B uses test-time compute more effectively: on BRIGHT, its performance consistently increases with longer and more information-rich rewritten queries; it continues to outperform other retrievers when combined with an LLM reranker. Our training recipe is general and can be easily extended to future LLMs; to this end, we open-source our code, data, and model.

==> pages/app-pages/app-downsream-results.tex <==
\section{Additional Downstream Results}\label{app:downstream-results}

We present the results on MMLU and GPQA in Table~\ref{tab:main_nlp}.

\begin{table}[t]
    \centering
    % \resizebox{\textwidth}{!}{%
    \begin{tabular}{lccc}
    \toprule
        Retriever & Query Type & MMLU & GPQA  \\
    \midrule
        % \rowcolor{gray!10} 
        Closed-book & - & 71.1 & 31.3 \\       
        \midrule
        Contriever & Original question & 72.0 & 36.4 \\
        GRIT-7B & Original question & 74.1 & 32.3 \\
        Search Engine & Original question & - & 33.8 \\
        \textbf{\modelname} & Original question & 75.0 & \textbf{38.4} \\
        
        \midrule
        
        Contriever & \reasonq & 72.8 & 31.3 \\
        GRIT-7B & \reasonq & 74.7 & 30.8 \\
        Search Engine & \reasonq & - & 36.4 \\
        \textbf{\modelname} & \reasonq & \textbf{75.6} & 35.4 \\
    \bottomrule
    \end{tabular}
    % }
    \caption{Performance on NLP tasks where the knowledge sources are unknown or unavailable. 
    }
    \label{tab:main_nlp}
\end{table}


==> pages/app-pages/app-related-works.tex <==
\section{Additional Related Works}\label{app:related-work}

\paragraph{Test-time scaling for RAG.} Optimal test-time scaling~\citep{snell2024scaling}, which significantly increases the quality and efficiency of LLMs, requires balancing the compute across various components. Prior work has explored enhancing RAG at test time from the perspective of (1) \emph{Datastore scaling} by increasing its size and diversity~\citep{shao2024scaling}; (2) \emph{Context-length scaling} by increasing the number of retrieved documents in the context~\citep{jiang2024longrag, xu2023retrieval, yue2024inference}; (3) \emph{Reranker scaling} by increasing the number of top candidate documents to rerank and increasing the number of thinking tokens to rerank documents after retrieval~\citep{weller2025rank1}; (4) \emph{Iteration scaling} by increasing the number of rounds to retrieve and respond~\citep{trivedi2022interleaving, yue2024inference}. Our work studies the test-time scaling for RAG from a 5th perspective---\textit{rewriter scaling}---and highlights the benefit of allocating more test-time compute for rewriting queries~\citep{liu2024query, ma2023query} with reasoning, which critically affects the retrieval quality~\citep{su2024bright}.
